Sampling Equilibria: Fast No-Regret Learning in Structured Games

Learning and equilibrium computation in games are fundamental problems across computer science and economics, with applications ranging from politics to machine learning. Much of the work in this area revolves around a simple algorithm termed \emph{randomized weighted majority} (RWM), also known as "Hedge" or "Multiplicative Weights Update," which is well known to achieve statistically optimal rates in adversarial settings (Littlestone and Warmuth '94, Freund and Schapire '99). Unfortunately, RWM comes with an inherent computational barrier: it requires maintaining and sampling from a distribution over all possible actions. In typical settings of interest the action space is exponentially large, seemingly rendering RWM useless in practice. In this work, we refute this notion for a broad variety of \emph{structured} games, showing it is possible to efficiently (approximately) sample the action space in RWM in \emph{polylogarithmic} time. This gives the first efficient no-regret algorithms for problems such as the \emph{(discrete) Colonel Blotto game}, \emph{matroid congestion}, \emph{matroid security}, and basic \emph{dueling games}. As an immediate corollary, we give a polylogarithmic time meta-algorithm to compute approximate Nash Equilibria for these games that is exponentially faster than prior methods in several important settings. Further, our algorithm is the first to efficiently compute equilibria for more involved variants of these games with general sums, more than two players, and, for Colonel Blotto, multiple resource types.

==> OH-hypergraph.tex <==
\subsection{Linear Hypergraph Game} All the games that we consider fall under the following class of game which we denote as the \emph{Linear Hypergraph Game}. Formally, we consider games played over $k$-uniform hypergraphs ${\Omega \choose k}$ whose rewards are \textit{linear} over the vertices in the following sense.
\begin{definition}[Linear Hypergraph Game]
Let $\mathcal{I}=(\{\Omega_i\}_{i=1}^m,\{R_i\}_{i=1}^m\}$ be an $m$-player game and $i$ an index such that $\Omega_i \subset {\Omega \choose k}$ for some ground set $\Omega$ and $k \in \mathbb{N}$. We say $\Omega_i$ is linear with respect to $\mathcal{I}$ if there exists a `vertex-wise' reward matrix $R^\Omega_i$ such that for all $t_1,\ldots,t_n \in \Omega_1 \times \ldots \times \Omega_n$
\[
R_i(t_1,\ldots,t_m) = \sum\limits_{v \in t_i} R^\Omega_i(t_1,\ldots, t_{i-1},v,t_{i+1},\ldots, t_m).
\]
\end{definition}
\noindent In other words, each element $v$ in the ground set $\Omega$ has a certain reward with respect to any choices of the opponents, and the reward of a $k$-set is simply the sum of its individual rewards. \maxh{Note similar settings considered in prior literature? Namely the component hedge paper.}

\paragraph{Optimistic Hedge} We are interested in designing efficient no-regret learning algorithms for many important games that fall under this class. The high-level algorithmic framework is the Optimistic Hedge, a variant of the multiplicative-weights-updates which is frequently applied in the setting of no-regret learning in games. For player $i \in [m]$, the Optimistic Hedge (OH) chooses the mixed strategy $\delta\lp( \Omega_i \rp)$ as follows: at the $1$st round, it chooses the uniform strategy $x^{(1)} = (1/ \abs{\Omega_i}, \cdots, 1 / \abs{\Omega_i} )$. At the $(T+1)$-th round, given the strategy history of the other players as $s_j^{(t)}$ for $j \in [m] \backslash \{i\}$ and $t \in [T]$.
For all $T$, a cumulative reward is computed for each strategy $x \in \Omega_i$
$$
r^{(T+1)}(x) = \sum_{t=1}^T R_i(s_1^{(t)}, \cdots, s_{i-1}^{(t)}, x, s_{i+1}^{(t)}, \cdots, s_m^{(t)}).
$$
Then, Optimistic Hedge chooses the mixed strategy $OH(T+1)$, which we denote as the Optimistic Hedge Distribution, such that 
\begin{align}
\label{eq:OH-def}
\Pr\lp[ OH(T+1) = x \rp] \propto r^{(T+1)}(x).
\end{align}
In the work of \cite{daskalakis2021near}, it has been show that, one can achieve a regret bound of $\polylog(T)$ in multi-player general sum game (if all players play according to the Optimistic Hedge Rule), and $\sqrt{T}$ for adversarial regret if the agent plays according to the Optimistic Hedge Rule \emph{exactly}. Exact sampling from distributions with exponentially large support is arguably a difficult algorithmic task and can be shown to be $\#P$-hard in many cases. Nonetheless, we show that similar regret bounds hold even when one implements Optimistic Hedge \emph{approximately}. \maxh{Give the adversarial bound as well.}
\begin{lemma}
\label{lem:apx_omwu}
For $\delta > 0$, if all players ($m$ total) sample from a distribution within $\delta$-TV distance of OMWU in each round $t=1,...,T$, then the regret of a player $i \in [m]$ with $n_i$ experts and maximum loss $\Lmax$ is bounded by
\begin{align*}
    \Reg_{i,T} \leq O\rbrac{m \Lmax n_i \log^4 T + \delta \Lmax T + \delta \Lmax^2 T^2}.
\end{align*}
\end{lemma}
\noindent As an immediate corollary, we get an efficient no-regret algorithm for any linear hypergraph game whose state space can be approximately sampled.
In the following two sections, we develop two different types of method of approximate sampling from the Optimistic Hedge Distribution in many well-studied settings in game theory and show how such results lead to new efficient no-regret learning algorithms for these games.

==> backup-cce.tex <==
\section{Computing CCE}
\begin{algorithm}[H]
\caption{Sampling-Hedge-MWU} \label{alg:cce-compute}
\begin{algorithmic}[1]
\Require The reward functions $R_i$. Sample Size $\lambda \in Z^+$.
\State Initialize the MWU distribution $\tilde s^{(0)}_i$ as the uniform distribution.
\For{$t=1 \cdots T$}
\For{$i=1 \cdots m$}
% \State Let $s_i^{(t)}$ be the MWU mixed strategy defined with respect to the strategy histories $ S_{-i}$.
\State Let $\tilde s_i^{(t)} = \textbf{MWU-Sampler}\lp( \bigg\{v_{j}^{(t',\tau)} \bigg | \text{ for } t' < t, j \in [m] \backslash \{i\}, \tau \in \lambda \bigg\} \rp)$ .\\
\Comment{$\tilde s_i^{(t)}$ is $f(\lambda)$ close to $s_i^{(t)}$, where $s_i^{(t)}$ is the exact MWU distribution updated according to $\tilde s_{-i}^{(t')}$ for $t' < t$.} \\
\State $\delta$ approximate sample $ v_i^{(t, 1)}, \cdots, v_i^{(t, \lambda)}$ from $\tilde s_i^{(t)}$.\\
\Comment{For $\tilde s_i^{(t)}$, the reward function is $O(\lambda t)$ piecewise constant, and computes the succinct description takes time probably $ O(m \lambda t) $.} \\
\Comment{$\delta$-approximate sample from $\tilde s_i^{(t)}$ can be done in time $\poly(m \lambda t / \delta,C)$, where $C$ depends on the game.}
\EndFor
\EndFor
\Comment{$\frac{1}{T}  \tilde s_1^{(t)} \otimes \cdots \otimes \tilde s_m^{(t)}$ is a $f(\lambda, \delta, T)$-approximate CCE.}
\For{$j = 1 \cdots \zeta$}
\State Sample $t \in [T]$ uniformly, then ($\delta'$-approximate) sample $v_i^{(j)}$ from $\tilde s_i^{(t)}$ for $i \in [m]$.
\EndFor
\State \Return 
$ \frac{1}{\zeta} \sum_{j=1}^{\zeta} v_1^{(j)} \otimes \cdots \otimes v_m^{(j)}  $.
\end{algorithmic}
\end{algorithm}
With a slight abuse of notation, we will also use $\tilde s_i^{(t)}$ to denote the mixed strategy from which the sampler is sampling if one sets $\delta = 0$ (namely, the exact MWU distribution with respect to the $\{ v_j^{(t', \tau)} \}$).
\begin{lemma}
\label{lem:sample-hedge-tv-dist}
Let $s_i^{(t)}$ be the MWU distribution with respect to the expected reward $ \sum_{t'=1}^t R_i\lp( e_i, \tilde s_{-i}^{(t')}  \rp) $ for each $e_i \in \Actions_i$. 
For any $\eps \in (0,1)$.
Assuming $$\lambda = C \cdot T^2 \Lmax^2 \cdot \log (mTN) / \eps^2, \,\text{ and } \delta \leq \sqrt{  \log(mtN) / \lambda }$$
for sufficiently large constant $C$.
Then, for all $i \in [m], t \in [T]$, 
it holds 
$
\TV \lp( \tilde s_i^{(t)}, s_i^{(t)} \rp)
\leq \eps
$
with probability at least $9/10$.
\end{lemma}
\begin{proof}
Fix a player $i \in [m]$, a strategy $e_i \in \Actions_i$ and a iteration $t$, 
we argue that  
\begin{align}
\label{eq:reward-concentration}
    \abs{ R(e_i, \tilde s_{-i}^{(t)} ) - \frac{1}{\lambda} \cdot \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} )  }
    \leq O \lp(\Lmax \cdot \sqrt{ \log( m T N ) /\lambda } \rp) \eqdef \kappa
\end{align}
with probability at least $1/(mTN)$.

Recall that $v_{-i}^{t, \tau}$ are sampled from some distribution $D$ that is within $\delta$ TV distance from $\tilde s_{-i}^{(t)}$.
Hence, we have that 
\begin{align}
 \abs{\E \lp[ \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) \rp]   
 - \lambda \cdot R(e_i, \tilde s_{-i}^{(t)} )}
 \leq \lambda \cdot \Lmax \cdot \delta. 
\end{align}
By Hoeffding's Inequality, for all $\xi > 0$ we have that
\begin{align}
\Pr \lp[ 
    \abs{   \E \lp[ \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) \rp] - \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) }
    \geq \xi
    \rp] \leq 
    2 \exp \lp( 
    \frac{ 2 \xi^2 }{\lambda \cdot \Lmax^2} \rp).
\end{align}
Set $\xi \eqdef C \cdot \sqrt{ \log( m T N ) \lambda } \Lmax$ for some constant $C$ then gives us
\begin{align}
    \abs{   \E \lp[ \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) \rp] - \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) }
    \leq C \cdot \sqrt{ \log( m T N ) \lambda } \Lmax
\end{align}
with probability at least $1 - \frac{1}{mTN}$.
By triangle's inequality, we have that 
\begin{align}
    \abs{    
    \lambda \cdot R(e_i, \tilde s_{-i}^{(t)})
    - \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) }
    \leq C \cdot \sqrt{ \log( m T N ) \lambda } \Lmax
    + \lambda \cdot \Lmax \cdot \delta
\end{align}
with probability at least $1 - \frac{1}{mTN}$. Dividing both sides by $\lambda$ then gives us
\begin{align}
    \abs{    
     R(e_i, \tilde s_{-i}^{(t)})
    - \frac{1}{\lambda} \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t, \tau} ) }
    \leq O \lp(\Lmax \cdot \sqrt{ \log( m T N ) /\lambda } \rp).
\end{align}
with probability at least $1 - \frac{1}{mTN}$.
By union bound, we have Equation~\eqref{eq:reward-concentration} holds for $i, e_i, t$ with probability at least $9/10$.
Condition on that, for all $t \in T, i \in [m]$ we have
\begin{align}
    \abs{ 
    \sum_{t' \leq t} R(e_i, \tilde s_{-i}^{(t')} ) - \sum_{t' \leq t} \frac{1}{\lambda} \cdot \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t', \tau} )  
    }
    \leq \kappa \cdot T.
\end{align}
Recall that $s_i^{(t)}$ is the mixed strategy where
$$
\Pr \lp[ s_i^{(t)} = e_i \rp] \propto 
\exp \lp( \log \beta \cdot \sum_{t' \leq t} R(e_i, \tilde s_{-i}^{(t')} ) \rp) \eqdef w_{i}^{(t)}(e_i).
$$
and $\tilde s_i^{(t)}$ is the mixed strategy where
$$
\Pr \lp[ \tilde s_i^{(t)} = e_i \rp] \propto 
\exp \lp( \log \beta  \cdot \lp( \sum_{t' \leq t} \frac{1}{\lambda} \cdot \sum_{\tau = 1}^{\lambda} R(e_i, v_{-i}^{t', \tau} ) \rp)   \rp) \eqdef \tilde w_{i}^{(t)}(e_i).
$$
We have  $\tilde w_i^{(t)}(e_i)$  is a $\rho$-approximation of  $w_i^{(t)}(e_i)$ where
\begin{align}
    \rho \eqdef \exp\lp( \log \beta \cdot \kappa \cdot T \rp)
    =  \exp \lp( O \lp(T \Lmax \cdot \sqrt{ \log( m T N ) /\lambda } \rp)  \rp).
    \leq O \lp(T \Lmax \cdot \sqrt{ \log( m T N ) /\lambda } \rp) \, ,
\end{align}
where the last inequality follows from $\exp(x) \leq 10 x$ for $x < 1$ and the fact that $\lambda = C \cdot T^2 \Lmax^2 \cdot \log (mTN)$ for sufficiently large constant $C$.
For all $i \in [m], t \in [T]$ we then have  
$$
\TV \lp( \tilde s_i^{(t)}, s_i^{(t)} \rp)
\leq O \lp(T \Lmax \cdot \sqrt{ \log( m T N ) /\lambda } \rp)
$$
with probability at least $9/10$ since the normalization operation preserves multiplicative approximations.
\end{proof}
\begin{definition}
For the $i$-th player, 
we say a sequence of (mixed) strategies $\{ s_i^{(1)}, \cdots, s_i^{(T)} \}$ have $\eps$ regret against another sequence of (mixed) strategies tuples 
$\{ s_{-i}^{(1)}, \cdots, s_{-i}^{(T)} \}$ if 
$$
\max_{ a_i \in \Actions_i }
 \sum_{t=1}^T R( a_i, s_{-i}^{(t)} )
 -
\sum_{t=1}^T R( s_i^{(t)}, s_{-i}^{(t)} )
 \leq \eps.
$$
\end{definition}
\begin{claim}
\label{clm:approx-mwu}
Suppose the sequence of strategies $\{ x_i^{(1)}, \cdots, x_i^{(T)} \}$ have $\eps_1$ regret against
$\{  x_{-i}^{(1)}, \cdots,  x_{-i}^{(T)} \}$. Let $\{ y_i^{(1)}, \cdots, y_i^{(T)} \}$ be another sequence of strategies satisfying that
$\TV \lp( x_i^{(t)}, y_i^{(t)} \rp) \leq \eps_2$.
Then, $\{ y_i^{(1)}, \cdots, y_i^{(T)} \}$ have regret $\eps_1 + \eps_2 \cdot T \Lmax$ against $\{  x_{-i}^{(1)}, \cdots,  x_{-i}^{(T)} \}$.
\end{claim}

\begin{lemma}[Original MWU Lemma]
\label{lem:vanila-mwu}
Let $s_i^{(t)}$ be the MWU distribution with respect to the expected reward $\sum_{t'=1}^t R_i\lp( e_i, \tilde s_{-i}^{(t')}  \rp) $ for each $e_i \in \Actions_i$. Then, it holds that $\{ s_i^{(1)}, \cdots, s_i^{(T)} \}$ has $O( \Lmax \cdot \sqrt{ \log N \cdot  T}   )$ regret against 
$\{ \tilde s_{-i}^{(1)}, \cdots, \tilde s_{-i}^{(T)} \}$.
\end{lemma}

\begin{lemma}
For any $\eps \in (0,1)$, assuming that 
$$
T = C_1 \cdot \Lmax^2 \cdot \log N / \eps^2, 
\lambda = C_2 \cdot T^4 \cdot \Lmax^4 \cdot \log( m T N ) / \eps^2,
\delta = \sqrt{ \log(mtN) / \lambda}.
$$
for sufficiently large constants $C_1, C_2$.
For any $i \in [m]$, the sequence of strategies $\{ \tilde s_i^{(1)}, \cdots, \tilde s_i^{(T)} \}$
has regret $\eps$ against $\{ \tilde s_{-i}^{(1)}, \cdots, \tilde s_{-i}^{(T)} \}$ with probability at least $9/10$.
In particular, this implies that 
$$
\sum_{t=1}^T  \tilde s_{1}^{(t)} \otimes  \cdots \otimes \tilde s_{m}^{(t)}
$$
composes of an $\eps$-CCE equilibrium.
\end{lemma}
\begin{proof}
Let $s_i^{(t)}$ be the MWU distribution with respect to the expected reward $ \sum_{t'=1}^t R_i\lp( e_i, \tilde s_{-i}^{(t')}  \rp) $ for each $e_i \in \Actions_i$. 
Setting $T = C_1 \cdot \Lmax^2 \cdot \log N / \eps^2$. 
Then, by Lemma~\ref{lem:vanila-mwu}, we have that $\{ s_i^{(1)}, \cdots, s_i^{(T)} \}$ has $\eps/2$ regret against 
$\{ \tilde s_{-i}^{(1)}, \cdots, \tilde s_{-i}^{(T)} \}$.
Setting $\lambda = C_2 \cdot T^4 \cdot \Lmax^4 \cdot \log( m T N ) / \eps^2,
\delta = \sqrt{ \log(mtN) / \lambda}$.  
Then, by Lemma~\ref{lem:sample-hedge-tv-dist}, 
we have that 
$\TV \lp( \tilde s_i^{(t)}, s_i^{(t)}\rp) \leq \eps / (2 T \Lmax)$ with probability at least $9/10$. 
Then, by Claim~\ref{clm:approx-mwu}, it then holds 
$\{ \tilde s_i^{(1)}, \cdots, \tilde s_i^{(T)} \}$ has $\eps$ regret against 
$\{ \tilde s_{-i}^{(1)}, \cdots, \tilde s_{-i}^{(T)} \}$ with probability at least $9/10$. 
\end{proof}

\begin{lemma}[CCE Compressing]
Let $\mathcal I = \{ \Actions_i, R_i\}$ be an $m$ player game.
Assume $\zeta = C \cdot \Lmax^2/\eps^2 \cdot \log(Nm)$ and $\delta = \eps / \Lmax$ for sufficiently large $C$.
Suppose $D \in \Delta \lp( \Actions_1 \otimes \cdots \otimes \Actions_m \rp)$ is an $\eps$-CCE of $\mathcal I$.
Let $(v_1^{(1)}, \cdots, v_m^{(1)}), \cdots, 
(v_1^{(\zeta)}, \cdots, v_m^{(\zeta)})$ be $\zeta$ pure strategy tuples sampled $\delta$-approximately from $D$. 
Then, 
$ \tilde D \eqdef \frac{1}{\zeta} \sum_{j=1}^{\zeta} v_1^{(j)} \otimes \cdots \otimes v_m^{(j)} $ composes of an $O(\eps)$-CCE of $\mathcal I$.
\end{lemma}
\begin{proof}
The fact that $D$ is an $\eps$-CCE of $\mathcal I$ gives us for any $j \in \zeta$ and any $i \in [m]$
\begin{align}
\label{eq:CCE-condition}
 \max_{e_i \in A_i } \E_{ (v_1, \cdots v_m) \sim D } \lp [ R_i( e_i, v_{-i} ) \rp]  - R_i(D) 
 \leq  \eps.    
\end{align}
We want to argue that for all $i \in m$, we simultaneously have
\begin{align}
\label{eq:CCE-def}
 \max_{e_i \in A_i } \E_{ (v_1, \cdots v_m) \sim \tilde D } \lp [ R_i( e_i, v_{-i} ) \rp]  - R_i(\tilde D) 
 \leq  O(\eps).    
\end{align}
with probability at least $9/10$.
This immediately implies that $\tilde D$ is an $O(\eps)$-CCE with probability at least $9/10$.

To argue Equation~\eqref{eq:CCE-def}, it suffices to show that  for each $i \in [m]$
\begin{align}
\label{eq:utility-concentrate}
    \abs{ R_i(\tilde D) - R_i(D) } 
    = \abs{   \frac{1}{\zeta} \sum_{j=1}^{\zeta} R_i \lp( v_1^{(j)}, \cdots, v_m^{(j)} \rp) -  R_i(D) }
    \leq O(\eps)
\end{align}
with probability at least $1 - 1/(20 m )$
and that for each $e_i \in A_i$
\begin{align}
\label{eq:action-utility-concentrate}
    \abs{ \E_{ (v_1, \cdots v_m) \sim \tilde D } \lp [ R_i( e_i, v_{-i} ) \rp]  - \E_{ (v_1, \cdots v_m) \sim  D } \lp [ R_i( e_i, v_{-i} ) \rp]  }
    =
    \abs{ \frac{1}{\zeta} \sum_{j=1}^{\zeta}  R_i( e_i, v_{-i}^{(j)} )  - \E_{ (v_1, \cdots v_m) \sim  D } \lp [ R_i( e_i, v_{-i} ) \rp]  }
    \leq O(\eps).
\end{align}
with probability at least $1 - 1/(20 N m )$.
We start with Equation~\eqref{eq:utility-concentrate}. Notice that  for each $j \in [\zeta]$ we have
$R_i \lp( v_1^{(j)}, \cdots, v_m^{(j)} \rp)$ are (i) independent, identically distributed (ii) within the interval $[-\Lmax, \Lmax]$, and (iii) satisfy
\begin{align}
    \E \lp[ 
     R_i \lp( v_1^{(j)}, \cdots, v_m^{(j)} \rp)
    \rp] = R_i(D) 
\end{align}
since the tuples $\lp( v_1^{(j)}, \cdots, v_m^{(j)} \rp)$ are sampled independently from $D$. Hence, Equation~\eqref{eq:utility-concentrate} follows from Hoeffding's Inequality with $\zeta \geq C \cdot \Lmax^2 / \eps^2 \cdot \log m $ for some sufficiently large constant $C$. The proof of Equation~\eqref{eq:action-utility-concentrate} is similar as long as
$\zeta \geq C \cdot \Lmax^2 / \eps^2 \cdot \log(Nm) $.

By union bound, we conclude that Equations~\eqref{eq:utility-concentrate}, \eqref{eq:action-utility-concentrate} hold simultaneously for all $i\in[m]$ and $e_i \in \Actions_i$ with probability at least $9/10$. 
Condition on that, Equations~\eqref{eq:utility-concentrate}, \eqref{eq:action-utility-concentrate} together with
Equation~\eqref{eq:CCE-condition} then give Equation~\eqref{eq:CCE-def} is true for all $i \in [m]$ simultaneously with probability at least $9/10$.
\end{proof}
\begin{proposition}
Let $\mathcal I$ be a game with $m$ player such that each action space size is bounded by $N$.
Suppose we have a \textbf{MWU-Sampler} that can performs $\delta$ approximate sample from the MWU distribution defined by $q$ pure strategy tuples in time 
$f(q, \delta)$ \footnote{The function should also depend on $m$, $N$. But those are game specific parameters.}.
Then, for any $\eps \in (0,1)$, there exists an algorithm \textbf{Sampling-Hedge} which outputs a $\eps$-approximate CCE of $\mathcal I$ in time 
$$
O\lp( 
T m \lambda \cdot f(T \lambda, \delta) 
+ \zeta m \cdot f(T \lambda, \delta')
\rp)
$$
where 
\begin{align*}
T &= C \cdot \Lmax^2 \cdot \log N / \eps^2, \\
\lambda &= C \cdot T^4 \cdot \Lmax^4 \cdot \log(mTN) / \eps^2, \\
\zeta &= C \Lmax^2 / \eps^2 \cdot \log(Nm), \\
\delta &= \sqrt{ \log(mtN) / \lambda }, \delta' = \eps / \Lmax.
\end{align*}
In other words, the runtime is
$$
O \lp( 
m  \cdot \Lmax^{14} \log^6 N / \eps^{12}
\cdot F \cdot \log(m\Lmax \log N / \eps )
\rp) \, ,
$$
where $F \eqdef f\lp( \Lmax^{14} \cdot \log^6 N / \eps^{12} \cdot \log(m \Lmax \log N / \eps ),   \frac{ \eps^5 }{  \Lmax^6 \cdot \log^2 N }  \rp)$ is the sampling cost.
\end{proposition}

==> exact.tex <==
Assume one is given pre-computed $f_h(y)$ for all $h \in [k]$ and $y \in [n] \cup \{0\}$, 
we would like to use them to design sampling procedure. 
% A subtle technical issue is that the probabilities are not necessarily rational numbers, which makes exact sampling difficult to perform.
% Nonetheless, 
% we argue that we can simply truncate everything after the first $\Theta( \log(nk / \delta) )$ digits for each $\Pr[x_{h+1} | x_{1 \cdots h}]$ and corresponding sampling procedure will yield a distribution that is still $\delta$ close to the exact MWU distribution in total variation distance.
% We will use $\fl_s( \cdot )$ to denote the function which truncates everything after the first $s$ digits after the decimal point.
\begin{lemma}
Let $e$ be the number of figures in $1/\beta$.
Assume 
one is given the values 
$ \beta^{-j} $ for $j \in \{0, \vect w_{\max} \cdot k\}$
and $ f_h(y) $ with respect to the $t$-th round for all $h \in [k]$ and $y \in [n] \cup \{0\}$. Then, sampling from the MWU distribution can be performed in time 
$\tilde O\Bigg( k \cdot 
\bigg( n + k \log n +  \vect w_{\max }  k  t \cdot e \bigg) 
\Bigg)$.\footnote{ $\tilde O$ hides the poly-logarithmic dependencies that come from the arithmetic multiplication operations, which take time $O(d \log d)$ for two numbers of length $d$.  }
\end{lemma}
\begin{proof}
Fix a partial assignment $\vect x_{1 \cdots h}$, 
let
\begin{align}
A \lp[y\rp] 
&= 
\beta^{ - \vect w_{h+1} \ell_{h+1}(y) } \cdot f_{k-h-1}\lp(n - \snorm{1}{ \vect x_{1 \cdots h} } - y\rp). \\
% \tilde A \lp[y\rp] 
% &= 
% \fl_{s}\lp( \beta^{ - \vect w_{h+1} \ell_{h+1}(y) } \rp) 
% \cdot 
% \fl_{s}\lp(  
% f_{k-h-1}\lp(n - \snorm{1}{ \vect x_{1 \cdots h} } - y\rp)
% \rp).
\end{align}
It is easy to see that $A$, after normalization, becomes exactly $\Pr \lp[\vect x_{h+1} = y|  \vect x_{1 \cdots h} \rp] $.
Besides,
each entry in $f_{k-h-1}(\cdot)$ contains at most 
$d \eqdef O(k \log n + \vect w_{\max} k t e)$ digits from Equation~\eqref{eq:partition-function}.. 
Hence, each entry in $A$ contains at most $O(d)$ digits and can be computed in time $\tilde O(d)$. As a result, sampling can be performed in time 
$\tilde O( n + k \log n + \vect w_{\max} k t e )$ for the $h$-th battlefield. Multiplying everything by $k$ gives the runtime of the entire sampling process.
% On the other hand, $\tilde A$ has the property that 
% (i) $\tilde A$ differs with $A$ by at most $O(\frac{\delta}{nk})$
% (ii) each entry in $\tilde A$ contains at most 
% $$
% d \eqdef O \lp( n + k \log n +  \vect w_{\max }  k  t + \log(1 / \delta) \rp)$$ digits. Property (ii) ensures that one can efficiently sample from the multinomial distributions $\tilde M$ whose probabilities are proportional to $\tilde A$ in time $O(d)$.
% Property (i) will ensure that this multinomial distribution $\tilde M$ is $\delta / k$ closed to the ideal distribution specified by $A$ in total variation distance. Using the closeness of the two multinomial distributions, we can then argue via induction that the final joint distributions over $\vec x_{1 \cdots k}$ yielded by sampling according to $\tilde A$ is $\delta$-close in total variation distance. 
\end{proof}
% As one can see, the factor $k \cdot \vect w_{\max} \cdot t$ in the runtime of the sampling phase comes from the fact that the probability distributions from which the algorithm sample can have elements whose masses are as light as $\exp \lp ( - \log(1/\beta) \cdot  k \cdot \vect w_{\max} \cdot t  \rp)$. 
% \begin{lemma}
% Assume the values $f_h(y)$ with respect to the $t$-th round are precomputed for all $h \in [k]$ and $y \in [n] \cup \{0\}$. Then, sampling from the MWU distribution can be performed in time $O\lp( n \cdot k^2 \cdot \vect w_{\max} \cdot t \rp)$.
% \end{lemma}
Next, we will show how we could use dynamic programming to precompute the table specifying  $ f_h(y)$ and $\beta^{-j}$. for $j \in \{0, \cdots, \vect w_{\max} k\}$.
\begin{lemma}
The values 
$ \beta^{-j} $ for $j \in \{0, \vect w_{\max} \cdot k\}$
and $ f_h(y) $ with respect to the $t$-th round for all $h \in [k]$ and $y \in [n] \cup \{0\}$ can be computed in time 
$\tilde O(n \cdot k \cdot \min(n, t) \cdot d + \vect w_{\max}^2 k^2 e)$ for $d = \Theta\lp(k \log n + \vect w_{\max} kt \cdot e \rp)$.
\end{lemma}
\begin{proof}
Notice that we have the following recursion
\begin{align}
    f_h(y) = \sum_{x=0}^y \beta^{- \vect w_h \ell_h(x)}
    \cdot f_{h-1} \lp( y - x \rp).
\end{align}
Hence, we can fill the dp table for $f_h(y)$ with $O(n^2 k)$ arithmetic operations. 
% We will show that, if one always keeps $s + \vect w_{\max} t k$ digits after the decimal points, one can accurately compute $\fl_s(f_h(y))$.
Besides, when $n$ is substantially larger than the other parameters $k,\eps$, the following observation about $\ell_h$ becomes useful.
\begin{observation}
At the $t$-th round, $\ell_h$ is a $(t+1)$-piecewise constant function.
\end{observation}
Using the observation, we can obtain a better algorithm for pre-computing $f_h(y)$ in the regime $n > t$.
In particular, one can compute the \emph{prefix-sum} of the partition function 
\begin{align}
F_h(y) = 
\begin{cases}
\sum_{i=0}^y f_h(y) \text{ for } y \geq 0 \, ,\\
0 \text{ otherwise.}\\
\end{cases}
\end{align}

Let $[a_{h,1}, b_{h,1}], \cdots, [a_{h,t+1}, b_{h,t+1}]$ be the $t+1$ segments on which $\ell_h$ is piece-wise constant (we always have $a_{h,1} = 0, b_{h,t+1} = n$). Then, we can rewrite the recursion as
\begin{align} \label{eq:segment-recursion}
    f_h(y) = \sum_{q=1}^{t+1} \beta^{- \vect w_h \ell_h(a_{h,q})}
    \cdot \lp( F_{h-1} \lp( y - a_{h,q} \rp) - F_{h-1} \lp( y - b_{h,q}-1 \rp) \rp)
\end{align}
Computing the segments $[a_{h,1}, b_{h,1}], \cdots, [a_{h,t+1}, b_{h,t+1}]$ 
and the prefix sums $F_h(y)$
for all battlefields $h$ both takes at most $O(nk)$ arithmetic operations. 
It is easy to see that all the numbers that may occur in the computation contain at most 
$d \eqdef \Theta\lp(k \log n + \vect w_{\max} kt \cdot e \rp)$ digits (as $\beta^{-j}$ and $f_h(y)$ contain at most $O(d)$ digits.)
Since each arithmetic operations take time at most $\tilde O(d)$, we can obtain an algorithm for pre-computing $f_h(y)$ in time 
$\tilde O\lp( n \cdot k \cdot \min \lp(n, t\rp) \cdot d \rp)$ at the $t$-th round.
Finally, as each $\beta^{-j}$ contain at most $O(\vect w_{\max} t e)$ digits. Computing them cost at most $\tilde O(\vect w_{\max}^2 t^2 e)$.
\end{proof}

% \begin{lemma}
% Assume $1/\beta$ has $e$ digits (which should be about). 
% There exists an algorithm which computes the values $\fl_s \lp( f_h(y) \rp)$ with respect to the $t$-th round for all $h \in [k]$ and $y \in [n] \cup \{0\}$, and $ \beta^{-j} $ for all $j \in \{0, \vect w_{\max} \cdot k\}$
% in time $O(n \cdot k \cdot \min(n,t))$.
% \end{lemma}


% \begin{lemma}
% There exists an algorithm which computes the values $f_h(y)$ with respect to the $t$-th round for all $h \in [k]$ and $y \in [n] \cup \{0\}$ in time $O(n \cdot k \cdot \min(n,t))$.
% \end{lemma}

==> meta_alg.tex <==
Recall that in the Colonel Blotto Game, a player tries to assign $n$ troops to $k$ battlefields. The player is said to win the battlefield $j \in [k]$ if she assigns strictly more troops to the battlefield than other players. As a result, she will earn an reward of $\vect w_j$. In MWU, players keep playing the games for $T$ rounds. 
At the $t$-th round, we will discuss how the first player could sample from the MWU distribution efficiently given the historic strategies (from round $1$ to $t-1$) of the other players.

Given an assignment $\vect x$, we will use $\ell_j(\vect x_j)$ to denote the number of times such that the assignment could win the $j$-th battlefield with respect to the historic strategies of all the other players. We will denote by $P_h: \Z^+ \mapsto \R^+$ for $h \in [k]$ the partition function defined as the following
\begin{align}
\label{eq:partition-function}
    f_h(y)
    = \sum_{ \vect x_1 + \cdots + \vect x_h = y } \prod_{i=1}^h \beta^{- \vect w_i \ell_i(\vect x_1) }.
\end{align}
Notice that $f_k(n)$ is precisely the normalization factor used in computing the MWU distribution. 
We remark that one can use the partition functions to sample from the MWU distribution. In particular, one samples the number of soldiers to put in each battlefield sequentially. One puts $\vect x_1 \in \{0, \cdots, n\}$ soldier to the first battlefield with probability
\begin{align} \label{eq:partition-sample-base}
\Pr[\vect x_1 = y] \propto
\beta^{ - \vect w_1 \ell_1(y) } \cdot f_{k-1}(n - y).
% =
% \frac{ \beta^{ - \vect w_1 \ell_1(y) } \cdot f_{k-1}(n - y)}
% { \sum_{z=0}^n \beta^{ - \vect w_1 \ell_1(z) } \cdot f_{k-1}(n - y)}
\end{align}
To sample from the $(h+1)$-th battlefield condition on that one has put $\vect x_1, \cdots, \vect x_{h}$ soldiers in the previous battlefields, one samples according to the distribution
\begin{align}
\label{eq:partition-sample-recursive}
\Pr \lp[\vect x_{h+1} = y|  \vect x_{1 \cdots h} \rp] 
\propto 
\beta^{ - \vect w_{h+1} \ell_{h+1}(y) } \cdot f_{k-h-1}\lp(n - \snorm{1}{ \vect x_{1 \cdots h} } - y\rp)  .
\end{align}
Notice that the probabilities defined according to Equations 
~\eqref{eq:partition-sample-base},~\eqref{eq:partition-sample-recursive}  yields exactly the MWU distribution. 

==> todo.tex <==
1. complete blotto results
2. move bit complexity stuff to appendix
3. write corollaries for DP games in section 5
4. write corollaries for MCMC games in section 6
5. table for intro
6. writeup approximate OMWU argument
7. generalize the dueling games
